SlimSeiz: Efficient Channel-Adaptive Seizure Prediction Using a Mamba-Enhanced Network

Epileptic seizures cause abnormal brain activity, and their unpredictability can lead to accidents, underscoring the need for long-term seizure prediction. Although seizures can be predicted by analyzing electroencephalogram (EEG) signals, existing methods often require too many electrode channels or larger models, limiting mobile usability. This paper introduces a SlimSeiz framework that utilizes adaptive channel selection with a lightweight neural network model. SlimSeiz operates in two states: the first stage selects the optimal channel set for seizure prediction using machine learning algorithms, and the second stage employs a lightweight neural network based on convolution and Mamba for prediction. On the Children's Hospital Boston-MIT (CHB-MIT) EEG dataset, SlimSeiz can reduce channels from 22 to 8 while achieving a satisfactory result of 94.8% accuracy, 95.5% sensitivity, and 94.0% specificity with only 21.2K model parameters, matching or outperforming larger models' performance. We also validate SlimSeiz on a new EEG dataset, SRH-LEI, collected from Shanghai Renji Hospital, demonstrating its effectiveness across different patients. The code and SRH-LEI dataset are available at https://github.com/guoruilu/SlimSeiz.

==> tables/ch_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Impact of Channel Count on Performance Metrics (Accuracy, Sensitivity, Specificity)}% For most patients, the accuracy corresponding to 4 channels is already above 90\%, and increasing channel numbers doesn't result in significant imrpovement. For the patients whose accuracy is below 90\%, increasing channels number has a positive effect on performance.}
\label{tab:ch_res}
\resizebox{1.95\columnwidth}{!}{%
\begin{tabular}{cccclccclccclccc}
\toprule[1pt]
        & \multicolumn{3}{c}{4ch}  &  & \multicolumn{3}{c}{6ch}  &  & \multicolumn{3}{c}{8ch}  &  & \multicolumn{3}{c}{10ch} \\ \cline{2-4} \cline{6-8} \cline{10-12} \cline{14-16} 
        & acc    & sens   & spec   &  & acc    & sens   & spec   &  & acc    & sens   & spec   &  & acc    & sens   & spec   \\ \cline{1-4} \cline{6-8} \cline{10-12} \cline{14-16} 
1       & 0.9804 & 0.9809 & 0.9800 &  & 0.9835 & 0.9816 & 0.9854 &  & 0.9856 & 0.9842 & 0.9871 &  & 0.9824 & 0.9830 & 0.9818 \\
2       & 0.9431 & 0.9531 & 0.9329 &  & 0.9628 & 0.9922 & 0.9333 &  & 0.9664 & 0.9913 & 0.9412 &  & 0.9671 & 0.9908 & 0.9432 \\
3       & 0.9745 & 0.9904 & 0.9585 &  & 0.9767 & 0.9863 & 0.9671 &  & 0.9825 & 0.9938 & 0.9711 &  & 0.9832 & 0.9881 & 0.9783 \\
4       & 0.9832 & 0.9906 & 0.9758 &  & 0.9884 & 0.9958 & 0.9809 &  & 0.9870 & 0.9948 & 0.9791 &  & 0.9893 & 0.9933 & 0.9852 \\
5       & 0.8280 & 0.9280 & 0.7278 &  & 0.8531 & 0.8889 & 0.8172 &  & 0.8803 & 0.9263 & 0.8341 &  & 0.8939 & 0.9268 & 0.8611 \\
6       & 0.8530 & 0.8204 & 0.8857 &  & 0.8574 & 0.8251 & 0.8897 &  & 0.8577 & 0.8453 & 0.8701 &  & 0.8635 & 0.8275 & 0.8996 \\
7       & 0.9696 & 0.9708 & 0.9684 &  & 0.9870 & 0.9953 & 0.9785 &  & 0.9879 & 0.9962 & 0.9795 &  & 0.9895 & 0.9934 & 0.9856 \\
8       & 0.8873 & 0.9063 & 0.8683 &  & 0.9203 & 0.9598 & 0.8808 &  & 0.9321 & 0.9681 & 0.8960 &  & 0.9351 & 0.9640 & 0.9063 \\
9       & 0.9551 & 0.9830 & 0.9272 &  & 0.9612 & 0.9703 & 0.9521 &  & 0.9681 & 0.9906 & 0.9455 &  & 0.9751 & 0.9832 & 0.9670 \\
10      & 0.9106 & 0.9516 & 0.8694 &  & 0.9184 & 0.9480 & 0.8887 &  & 0.9300 & 0.9646 & 0.8954 &  & 0.9322 & 0.9501 & 0.9142 \\
11      & 0.9946 & 0.9992 & 0.9901 &  & 0.9950 & 0.9998 & 0.9902 &  & 0.9955 & 0.9995 & 0.9916 &  & 0.9950 & 0.9990 & 0.9911 \\
12      & 0.8224 & 0.8187 & 0.8262 &  & 0.8434 & 0.8343 & 0.8524 &  & 0.8504 & 0.8255 & 0.8752 &  & 0.8668 & 0.8930 & 0.8406 \\
13      & 0.9402 & 0.9745 & 0.9059 &  & 0.9361 & 0.9761 & 0.8961 &  & 0.9408 & 0.9728 & 0.9087 &  & 0.9418 & 0.9807 & 0.9028 \\
14      & 0.9270 & 0.8635 & 0.9903 &  & 0.9282 & 0.8705 & 0.9858 &  & 0.9288 & 0.8613 & 0.9963 &  & 0.9287 & 0.8748 & 0.9825 \\
15      & 0.8181 & 0.7979 & 0.8383 &  & 0.8482 & 0.7805 & 0.9160 &  & 0.9329 & 0.8863 & 0.9795 &  & 0.9334 & 0.8962 & 0.9706 \\
16      & 0.8447 & 0.9012 & 0.7882 &  & 0.8666 & 0.8939 & 0.8393 &  & 0.8631 & 0.9086 & 0.8176 &  & 0.8739 & 0.8806 & 0.8672 \\
17      & 0.9774 & 0.9820 & 0.9728 &  & 0.9745 & 0.9868 & 0.9622 &  & 0.9793 & 0.9814 & 0.9771 &  & 0.9827 & 0.9951 & 0.9703 \\
18      & 0.9828 & 0.9935 & 0.9721 &  & 0.9877 & 0.9948 & 0.9806 &  & 0.9893 & 0.9933 & 0.9853 &  & 0.9896 & 0.9963 & 0.9828 \\
19      & 0.9964 & 0.9985 & 0.9944 &  & 0.9962 & 0.9973 & 0.9950 &  & 0.9967 & 0.9969 & 0.9965 &  & 0.9994 & 0.9998 & 0.9990 \\
20      & 0.9556 & 0.9746 & 0.9366 &  & 0.9623 & 0.9753 & 0.9493 &  & 0.9581 & 0.9719 & 0.9442 &  & 0.9636 & 0.9825 & 0.9447 \\
21      & 0.8501 & 0.9066 & 0.7935 &  & 0.8932 & 0.9373 & 0.8489 &  & 0.9129 & 0.9281 & 0.8976 &  & 0.9262 & 0.9786 & 0.8736 \\
22      & 0.9372 & 0.9622 & 0.9118 &  & 0.9433 & 0.9735 & 0.9127 &  & 0.9573 & 0.9794 & 0.9349 &  & 0.9577 & 0.9672 & 0.9480 \\
23      & 0.9316 & 0.9480 & 0.9152 &  & 0.9629 & 0.9738 & 0.9520 &  & 0.9625 & 0.9867 & 0.9384 &  & 0.9669 & 0.9893 & 0.9446 \\
24      & 0.9225 & 0.8809 & 0.9641 &  & 0.9302 & 0.8844 & 0.9758 &  & 0.9262 & 0.8880 & 0.9645 &  & 0.9252 & 0.8713 & 0.9790 \\
\hline
Average & 0.9244 & 0.9365 & 0.9122 &  & 0.9365 & 0.9426 & 0.9304 &  & 0.9446 & 0.9515 & 0.9378 &  & 0.9484 & 0.9544 & 0.9425 \\ 
\bottomrule[1pt]
\end{tabular}%
}
\end{table*}
